Study of Cabibbo Suppressed Decays of the Ds Charmed-Strange Meson involving a KS

We study the decay of Ds meson into final states involving a Ks and report the discovery of Cabibbo suppressed decay modes Ds -> Kspi-pi+pi+ (179 +/- 36 events) and Ds -> Kspi+ (113 +/-26 events). The branching ratios for the new modes are Gamma(Ds -> Kspi-pi+pi+)/Gamma(Ds -> KsK-pi+pi+) = 0.18 +/- 0.04 +/- 0.05 and Gamma(Ds -> Kspi+)/Gamma(Ds -> KsK+) = 0.104 +/- 0.024 +/- 0.013.

==> e831latest.tex <==
\affiliation{University of California, Davis, CA 95616}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brasil}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\affiliation{University of Colorado, Boulder, CO 80309}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
\affiliation{University of Guanajuato, 37150 Leon, Guanajuato, Mexico}
\affiliation{University of Illinois, Urbana-Champaign, IL 61801}
\affiliation{Indiana University, Bloomington, IN 47405}
\affiliation{Korea University, Seoul, Korea 136-701}
\affiliation{Kyungpook National University, Taegu, Korea 702-701}
\affiliation{INFN and University of Milano, Milano, Italy}
\affiliation{University of North Carolina, Asheville, NC 28804}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\affiliation{Pontif\'\i cia Universidade Cat\'olica, Rio de Janeiro, RJ, Brazil}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\affiliation{University of South Carolina, Columbia, SC 29208}
\affiliation{University of Tennessee, Knoxville, TN 37996}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\affiliation{University of Wisconsin, Madison, WI 53706}
\author{J.~M.~Link}
\affiliation{University of California, Davis, CA 95616}
\author{P.~M.~Yager}
\affiliation{University of California, Davis, CA 95616}
\author{J.~C.~Anjos}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{I.~Bediaga}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{C.~Castromonte}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{A.~A.~Machado}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{J.~Magnin}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{A.~Massafferri}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{J.~M.~de~Miranda}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{I.~M.~Pepe}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{E.~Polycarpo}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{A.~C.~dos~Reis}
\affiliation{Centro Brasileiro de Pesquisas F\'\i sicas, Rio de Janeiro, RJ, Brazil}
\author{S.~Carrillo}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{E.~Casimiro}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{E.~Cuautle}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{A.~S\'anchez-Hern\'andez}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{C.~Uribe}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{F.~V\'azquez}
\affiliation{CINVESTAV, 07000 M\'exico City, DF, Mexico}
\author{L.~Agostino}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{L.~Cinquini}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{J.~P.~Cumalat}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{V.~Frisullo}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{B.~O'Reilly}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{I.~Segoni}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{K.~Stenson}
\affiliation{University of Colorado, Boulder, CO 80309}
\author{J.~N.~Butler}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{H.~W.~K.~Cheung}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{G.~Chiodini}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{I.~Gaines}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{P.~H.~Garbincius}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{L.~A.~Garren}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{E.~Gottschalk}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{P.~H.~Kasper}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{A.~E.~Kreymer}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{R.~Kutschke}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{M.~Wang}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\author{L.~Benussi}
\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
%\author{M.~Bertani}
%\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
\author{S.~Bianco}
\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
\author{F.~L.~Fabbri}
\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
%\author{S.~Pacetti}
%\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
\author{A.~Zallo}
\affiliation{Laboratori Nazionali di Frascati dell'INFN, Frascati, Italy I-00044}
\author{M.~Reyes}
\affiliation{University of Guanajuato, 37150 Leon, Guanajuato, Mexico}
\author{C.~Cawlfield}
\affiliation{University of Illinois, Urbana-Champaign, IL 61801}
\author{D.~Y.~Kim}
\affiliation{University of Illinois, Urbana-Champaign, IL 61801}
\author{A.~Rahimi}
\affiliation{University of Illinois, Urbana-Champaign, IL 61801}
\author{J.~Wiss}
\affiliation{University of Illinois, Urbana-Champaign, IL 61801}
\author{R.~Gardner}
\affiliation{Indiana University, Bloomington, IN 47405}
\author{A.~Kryemadhi}
\affiliation{Indiana University, Bloomington, IN 47405}
%\author{C.~H.~Chang}
%\affiliation{Korea University, Seoul, Korea 136-701}
\author{Y.~S.~Chung}
\affiliation{Korea University, Seoul, Korea 136-701}
\author{J.~S.~Kang}
\affiliation{Korea University, Seoul, Korea 136-701}
\author{B.~R.~Ko}
\affiliation{Korea University, Seoul, Korea 136-701}
\author{J.~W.~Kwak}
\affiliation{Korea University, Seoul, Korea 136-701}
\author{K.~B.~Lee}
\affiliation{Korea University, Seoul, Korea 136-701}
\author{K.~Cho}
\affiliation{Kyungpook National University, Taegu, Korea 702-701}
\author{H.~Park}
\affiliation{Kyungpook National University, Taegu, Korea 702-701}
\author{G.~Alimonti}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{S.~Barberis}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{M.~Boschini}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{A.~Cerutti}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{P.~D'Angelo}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{M.~DiCorato}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{P.~Dini}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{L.~Edera}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{S.~Erba}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{P.~Inzani}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{F.~Leveraro}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{S.~Malvezzi}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{D.~Menasce}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{M.~Mezzadri}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{L.~Moroni}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{D.~Pedrini}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{C.~Pontoglio}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{F.~Prelz}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{M.~Rovere}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{S.~Sala}
\affiliation{INFN and University of Milano, Milano, Italy}
\author{T.~F.~Davenport~III}
\affiliation{University of North Carolina, Asheville, NC 28804}
\author{V.~Arena}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{G.~Boca}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{G.~Bonomi}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{G.~Gianini}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{G.~Liguori}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{D.~Lopes~Pegna}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{M.~M.~Merlo}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{D.~Pantea}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{S.~P.~Ratti}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{C.~Riccardi}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{P.~Vitulo}
\affiliation{Dipartimento di Fisica Nucleare e Teorica and INFN, Pavia, Italy}
\author{C.~G\"obel}
\affiliation{Pontif\'\i cia Universidade Cat\'olica, Rio de Janeiro, RJ, Brazil}
\author{J.~Otalora}
\affiliation{Pontif\'\i cia Universidade Cat\'olica, Rio de Janeiro, RJ, Brazil}
\author{H.~Hernandez}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{A.~M.~Lopez}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{H.~Mendez}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{A.~Paris}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{J.~Quinones}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{J.~E.~Ramirez}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{Y.~Zhang}
\affiliation{University of Puerto Rico, Mayaguez, PR 00681}
\author{J.~R.~Wilson}
\affiliation{University of South Carolina, Columbia, SC 29208}
\author{T.~Handler}
\affiliation{University of Tennessee, Knoxville, TN 37996}
\author{R.~Mitchell}
\affiliation{University of Tennessee, Knoxville, TN 37996}
%\author{A.~D.~Bryant}
%\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{D.~Engh}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{M.~Hosack}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{W.~E.~Johns}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{E.~Luiggi}
\affiliation{Vanderbilt University, Nashville, TN 37235}
%\author{J.~E.~Moore}
%\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{M.~Nehring}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{P.~D.~Sheldon}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{E.~W.~Vaandering}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{M.~Webster}
\affiliation{Vanderbilt University, Nashville, TN 37235}
\author{M.~Sheaff}
\affiliation{University of Wisconsin, Madison, WI 53706}
\collaboration{The FOCUS Collaboration}
\affiliation{See \textrm{http://www-focus.fnal.gov/authors.html} for additional author information.}

